M4: Multi-generator, Multi-domain, and Multi-lingual Black-Box Machine-Generated Text Detection

Large language models (LLMs) have demonstrated remarkable capability to generate fluent responses to a wide variety of user queries. However, this has also raised concerns about the potential misuse of such texts in journalism, education, and academia. In this study, we strive to create automated systems that can detect machine-generated texts and pinpoint potential misuse. We first introduce a large-scale benchmark \textbf{M4}, which is a multi-generator, multi-domain, and multi-lingual corpus for machine-generated text detection. Through an extensive empirical study of this dataset, we show that it is challenging for detectors to generalize well on instances from unseen domains or LLMs. In such cases, detectors tend to misclassify machine-generated text as human-written. These results show that the problem is far from solved and that there is a lot of room for improvement. We believe that our dataset will enable future research towards more robust approaches to this pressing societal problem. The dataset is available at https://github.com/mbzuai-nlp/M4.

==> section/analysis.tex <==
\section{Data Collection and Analysis}
\label{sec:datasetanalysis}
\subsection{Prompt Diversity}
For each generator model, we carefully designed multiple (2-8) prompts in various styles, aiming to produce diverse outputs that are more aligned to divergent generations in real-world application scenarios. 
For example, on simple domains of \wikipedia and \wikihow, two prompts are applied. For \arxiv and \reddit using \chatgpt, we use five different prompts, and four different prompts for \peerread.
We generate varying tones of responses by prompts such as \textit{answer the question} (1) ``like I am five years old''; (2) ``in an expert confident voice''; (3) ``in a formal academic and scientific writing voice'' and etc. 
\tabref{tab:num-prompts} in \appref{sec:datasetanalysis} provides the statistics of prompts used in the data collection.


\begin{table*}[ht]
    \centering
    \small
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|ccccc|c}
    \toprule
      Domain$\downarrow$ & davinc-003 &  ChatGPT &  Cohere &  Dolly-v2 &  Bloomz &  Unique across domain \\
        \midrule
       wikipedia & 1 &   1 &     1 &       1 &     2 &  3 \\
          Reddit & 5 &   5 &     1 &       1 &     1 &  8 \\
         wikihow & 1 &   1 &     1 &       1 &     2 &  3 \\
        peerread & 4 &   4 &     4 &       4 &     4 &  4 \\
           arxiv & 1 &   5 &     1 &       1 &     2 &  8 \\
           \midrule
    baike/web QA & 1 &   1 &     Na &       Na &     Na &     1 \\
           RuATD & 1 &   1 &     Na &       Na &     Na &     1 \\
  True Fake news & 1 &   1 &     Na &       Na &     Na &     1 \\
       Urdu-news & Na &   1 &     Na &       Na &     Na &     1 \\
    id\_newspaper& Na &   1 &     Na &       Na &     Na &     1 \\
Arabic wikipedia & Na &    1 &     Na &       Na &     Na &     1 \\
\bottomrule
\end{tabular}}
    \caption{Statistics of prompts for different domains and LLMs. One prompt is used for non-English text and multiple prompts for English. The number of prompts for different domains vary as shown in the last column. Given a domain, some models can not follow all designed instructions, leading to less variety of prompts for some models.}
    \label{tab:num-prompts}
\end{table*}


\paragraph{Generator Hyper-parameters}
\tabref{tab:hyperparameters} shows hyper-parameters we set for various generators. 
In general, we follow the default setting, except for the length of new generations in order to satisfy the minimum character length of 1,000.
\begin{table*}[ht]
    \centering
    \small
    \resizebox{\textwidth}{!}{
    \addtolength{\tabcolsep}{-1pt}
        \begin{tabular}{ll|lllllHH}
        \toprule
        \textbf{Source/} & \textbf{Language} & \multicolumn{7}{c}{\textbf{Generator}} \\
        \textbf{Domain} &                   & Davinci003    & ChatGPT & Cohere & Dolly-v2 & BLOOMz & FlanT5 & LLaMa \\ \midrule
        Wikipedia & English                 & max\_tokens=1000        & max\_tokens=1000 & max\_tokens=1000 & \begin{tabular}[c]{@{}l@{}}min\_new\_tokens=300, \\ max\_new\_tokens=1000\end{tabular} 
        & default & - & Yuxia \\ \midrule
        Reddit ELI5 & English               & default & default & default & \multirowcellii{
        min\_new\_tokens=180 \\ \midrule
        max\_new\_tokens=600 }
 & min\_new\_tokens=180 & \begin{tabular}[c]{@{}l@{}}min\_len=50, \\ max\_len=200\end{tabular} & Osama \\ \midrule
        WikiHow & English                   & max\_tokens=2000 & default & default & \multirowcellii{
        min\_new\_tokens=200 \\ 
        max\_new\_tokens=1000 } & min\_new\_tokens=200 & - & Yuxia \\  \midrule
        PeerRead & English                  & default & default & default & default & min\_new\_tokens=150 & - & \begin{tabular}[c]{@{}l@{}}min\_len=50, \\ max\_len=400\end{tabular} \\ \midrule
        arXiv abstract & English            & max\_tokens=3000 & default & default & \multirowcellii{ min\_new\_tokens=180 \\ max\_new\_tokens=600 }
  & \begin{tabular}[c]{@{}l@{}}min\_new\_tokens=180,\\ max\_new\_tokens=420,\\ repitition\_penalty=1.15,\\ length\_penalty=10\end{tabular} & \begin{tabular}[c]{@{}l@{}}min\_len=50, \\ max\_len=200\end{tabular} & Osama \\ \midrule
        Baike/Web QA & Chinese              & default & default & - & - & - & - & - \\ \midrule
        RuATD & Russian & max\_tokens=1700 & default & - & - & - & - & - \\ \midrule
        Urdu-news & Urdu                    & - & temperature=0 & - & - & - & - & - \\ \midrule
        id\_newspapers\_2018 & Indonesian   & - & default & - & - & - & - & - \\ \midrule
        Arabic-Wikipedia & Arabic           & - & default & - & - & - & - & - \\ \midrule
        Bulgarian True \& Fake News & Bulgarian & max\_tokens=3000 & default & - & - & - & - & - \\ \bottomrule
        \end{tabular}
        }
    \caption{Hyperparameters used to generate data. We only specify parameter values that are different from defaults.}
    \label{tab:hyperparameters}
\end{table*}
\\
\\
\textit{\textbf{Prompts of \peerread}}
\begin{itemize}
    \item Please write a peer review for the paper of + title;
    \item Write a peer review by first describing what problem or question this paper addresses, then strengths and weaknesses, for the paper + title;
    \item Please write a peer review for the paper of + title, its main content is as below: + abstract;
    \item Write a peer review by first describing what problem or question this paper addresses, then strengths and weaknesses, for the paper + title, its main content is as below: + abstract.
\end{itemize}

\subsection{Data Cleaning and Quality}
\paragraph{Data Cleaning}
Naive indicators in text, such as multiple newlines in \wikihow and \arxiv, and bullet points of machine-generated text, might be used by detectors to distinguish text written by human or machine. This may discourage detectors to capture more generalized signals to make a distinction. 
Therefore, we remove all comas of the beginning of new lines and multiple newlines (``\n'') for \wikihow text written by human, and remove all variations of bullet points for \wikihow machine text.
For human \wikipedia, we remove all references (e.g., [1], [2]), all URLs, all multiple newlines and paragraphs whose length is less than 50 characters. 
For \arxiv human-written abstracts, we remove the newlines stemming from paper PDF conversion.



\paragraph{Data Quality}
Different from other tasks where the data quality can be quantified through the agreement between annotators over gold labels, we naturally obtain gold labels along with the collection of machine-generated text.
Therefore, we guarantee the data quality by randomly sampling 10-20 cases for each domain /generator and manually assessing the plausibility of generated texts.
% In some cases, we use BERTScore for automatic detection of prompts that produce bad generations and replacing them with better alternatives. 
This can effectively circumvent incoherent, disorganized, and illogical generations that are easy to distinguish from human-written ones due to improper prompts or hyper-parameters settings of generators (e.g., some generators repeat newly-generated snippets to satisfy the minimum setup of new tokens).
In addition, to mimic the human-written texts, we control the length of MGTs to imitate similar lengths as humans. 


\subsection{N-gram Analysis}
Texts written by human demonstrate larger vocabulary (unigram) and more diverse bigrams across all domains compared with any of the generators, in \tabref{tab:ngramanalysis}.
Combination of all generators has comparable word coverage with humans.
Comparing between domains, \wikipedia covers broader topics, resulting in the largest amount of unique unigrams, and then \wikihow and \reddit.
Since \arxiv and \peerread involve narrow topics, only  academic papers and peer reviews, leading to a smaller amount of uni- and bi-grams.
Among five large language models, Dolly-v2 exhibit the largest number of unique words and bigrams, followed by davinci, ChatGPT, Bloomz, and Cohere as the last.
We calculate the overlap of unique words between human and machine text by Jaccard’s similarity, and find most of them are between 20-35\%, and 10-20\% for unique 2-grams. 
This indicates the different word distribution by human and machines, offering distinguishable signals.


\begin{table*}[ht]
    \centering
    \small
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|rrrrrr|rrrrrr}
    \toprule
      & \multicolumn{6}{c|}{\textbf{Word (unigram)}} & \multicolumn{6}{c}{\textbf{bigrams}} \\
      Domain$\downarrow$ & Human & ChatGPT &  davinc-003 &  Cohere &  Dolly-v2 &  Bloomz & Human & ChatGPT &  davinc-003 &  Cohere &  Dolly-v2 &  Bloomz \\
        \midrule
       \wikipedia & 144,523 & 45,275 & 59,038 & 47,092 & 65,059 & 34,304 &
        1,000,870 & 295,007 & 400,072 & 258,210 & 385,074 & 141,328 \\
          \reddit &  69,406 & 27,403 & 33,292 & 24,134 & 36,173 & 28,794 &
        586,341 & 253,075 & 315,567 & 183,926 & 308,695 & 212,334 \\
         \wikihow &  84,651 & 49,723 & 47,307 & 29,062 & 46,743 & 40,082 & 
         820,026 & 501,998 & 457,188 & 243,356 & 357,007 & 277,770 \\
        \peerread &  24,317 & 11,314 &  7,693 &  8,812 & 29,851 & 11,597 & 
        225,007 & 102,638 & 51,636 & 61,310 & 230,282 & 92,858 \\
           \arxiv &  36,202 & 18,291 & 29,024 & 22,777 & 35,808 & 29,989 & 
           263,781 & 145,954 & 186,561 & 149,892 & 251,770 & 209,053\\
           \midrule
           All domains & 252,244 & 95,775 & 115,482 & 87,428 & 139,981 & 96,789 & 2,364,143 & 1,047,293 & 1,145,593 & 733,902 & 1,220,512 & 775,387\\
           \midrule
      All & 252,244 & \multicolumn{5}{c|}{275,455} & 2,364,143 & \multicolumn{5}{c}{3,074,950} \\
\bottomrule
\end{tabular}}
    \caption{Statistics of words and 2-grams of text from Human vs. Generators.}
    \label{tab:ngramanalysis}
\end{table*}

% sentiment analysis
% more subjective or objective; and logical or emotional

\subsection{Human Evaluation}
\label{sec:humanevaluation}
Given \reddit and \arxiv (\chatgpt) test sets, for each domain, we sampled the first 50 (human, machine) pairs and shuffled the 100 pieces of text into two groups.
In case of 'cheating' comparison, any two texts from the same pair will not be selected in the same group.
On \reddit, there are 29 pieces of text from human and 21 from machine for group one, and (21 human, 29 machine) for group two; and (human:26, machine:24) for \arxiv group one, (human:24, machine:26) for \arxiv group two. 
Six annotators are invited to label whether the text is written by human or machine.
Each rater annotates 17 unique examples for \reddit (finished by six annotators) and 25 examples for \arxiv (finished by four).

We calculate the accuracy, precision, recall and F1-score for human evaluation and compare with the XLM-R fine-tuned by \reddit or \arxiv (\chatgpt) training data. 
\begin{table}[ht!]
\centering
\resizebox{0.7\columnwidth}{!}{
    \begin{tabular}{l c c c c | c c c c}
        \toprule
        Domain$\rightarrow$ & \multicolumn{4}{c}{\textbf{\reddit}} & \multicolumn{4}{c}{\textbf{\arxiv}} \\
        Group$\downarrow$ & Accuracy & Prec & Recall & F1 & Accuracy & Prec & Recall & F1 \\
        \midrule
        XLM-R &  0.996 & 0.992 & 1.000 & 0.996 &  1.000 &  1.000 &  1.000 &  1.000 \\
        \midrule
        All & 0.770 & 0.770 & 0.770 & 0.770 & 0.720 & 0.739 & 0.720 & 0.714 \\
        Group1 & 0.780 & 0.775 & 0.771 & 0.773 & 0.720 & 0.744 & 0.713 & 0.708\\
        Group2 & 0.760 & 0.754 & 0.754 & 0.754 & 0.720 & 0.733 & 0.724 & 0.718 \\
        \midrule
        Annotator1 & 0.765 & 0.846 & 0.750 & 0.742 & 0.600 & 0.675 & 0.612 & 0.566 \\
        Annotator2 & 0.882 & 0.917 & 0.857 & 0.871 & 0.840 & 0.838 & 0.838 & 0.838 \\
        Annotator3 & 0.688 & 0.773 & 0.75 & 0.686 & 0.640 & 0.640 & 0.638 & 0.638  \\
        Annotator4 & 0.938 & 0.929 & 0.950 & 0.935 & 0.800 & 0.844 & 0.821 & 0.799 \\
        Annotator5 & 0.412 & 0.410 & 0.410 & 0.410 & -- & -- & -- & -- \\
        Annotator6 & 0.941 & 0.955 & 0.929 & 0.938 & -- & -- & -- & --\\
        
        \bottomrule
    \end{tabular}
    }
    \caption{Human evaluation on 100 examples from \reddit and \arxiv (human, \chatgpt). Fine-tuned XLM-R is much better than human.}
    \label{tab:human-eval}
\end{table}
% first_group_reddit_chatGPT:
% precision (machine text)    0.9820 (0.024648)
% recall (machine text)       1.0000
% f1 (machine text)           0.9908 (0.012598)
% accuracy                    0.9920 (0.012598)
% both_group_reddit_chatGPT:
% precision (machine text)    0.992 (0.010954)
% recall (machine text)       1.000
% f1 (machine text)           0.996 (0.005477)
% accuracy                    0.996 (0.005477)
% For all other test sets every metrics is 1 
Accuracy of human is 0.77 for \reddit and 0.72 for \arxiv, while the fined-tuned XLM-R shows close-to-one accuracy. This indicates it is not easy for human to distinguish, especially non-native English speakers who are also not familiar with the \chatgpt generation patterns (e.g., annotator 1,3,5).
Also, it is harder to distinguish text of \arxiv than \reddit.
We speculate that annotators can rely on less signals from the content but more by stylistic information to identify \arxiv text, leading to the accuracy gap between two domains.
Since it is challenging for general readers to understand and follow abstracts of academic papers, but it is easier to read \reddit answers.
% if removing the format signals, I find that human-written is shorter in each row when showing in the google sheet. if removing these, it will be more difficult, do we need to evaluate another version removing these format differences?





==> section/tables/acc_same_domain_across_generator.tex <==
\begin{table}[h]
    \centering
    \footnotesize
    \resizebox{0.49\columnwidth}{!}{
        \addtolength{\tabcolsep}{-1pt}
    \begin{tabular}{l  c  c  c c}
    \toprule
        % Test $\rightarrow$ & \multicolumn{4}{c|}{ChatGPT} & \multicolumn{4}{c|}{davinci} & \multicolumn{4}{c|}{Cohere} & \multicolumn{4}{c}{BLOOMz} \\
        Test $\rightarrow$ & ChatGPT & davinci & Cohere & BLOOMz \\
        Train $\downarrow$ & Acc & Acc & Acc & Acc \\
    \midrule
    \multicolumn{5}{c}{\textbf{RoBERTa(base)}} \\
    \midrule
        ChatGPT  &  \textbf{0.997} &  \textbf{0.997} &  0.994  &  0.777  \\
        davinci  &  0.996  &  0.995  &  0.994  &  0.814  \\
        Cohere  &  \textbf{0.997}  &  0.996  &  \textbf{0.996} &  0.826  \\
        BLOOMz  &  0.993  &  0.993  &  0.990  &  \textbf{0.981} \\
    \midrule
      \multicolumn{5}{c}{\textbf{ELECTRA(large)}} \\
    \midrule
        ChatGPT  &  \textbf{0.935} &  \textbf{0.918} &  0.836  &  0.566  \\
        davinci  &  0.886  &  0.887  &  0.838  &  0.624  \\
        Cohere  &  0.843  &  0.834  &  \textbf{0.855} &  0.724  \\
        BLOOMz  &  0.499  &  0.501  &  0.532  &  \textbf{0.975} \\
    \midrule
    \multicolumn{5}{c}{\textbf{LR-GLTR}} \\
    \midrule
        ChatGPT  &  0.963  &  0.653  &  0.969  &  0.655  \\
        davinci  &  0.812  &  \textbf{0.852}  &  0.785  &  0.737  \\
        Cohere  &  \textbf{0.968}  &  0.660  &  \textbf{0.970}  &  0.615  \\
        BLOOMz  &  0.892  &  0.712  &  0.795  &  \textbf{0.872}  \\
    \midrule
    \multicolumn{5}{c}{\textbf{Stylistic}} \\
    \midrule
        ChatGPT  &  \textbf{1.000}  &  0.710  &  0.877  &  0.624  \\
        davinci  &  0.973  &  \textbf{0.974}  &  0.828  &  0.871  \\
        Cohere  &  0.976  &  0.838  &  \textbf{0.988}  &  0.655  \\
        BLOOMz  &  0.634  &  0.760  &  0.555  &  \textbf{0.985}  \\
    \midrule
    \multicolumn{5}{c}{\textbf{NELA}} \\
    \midrule
        ChatGPT  &  \textbf{0.972}  &  0.520  &  0.642  &  0.488  \\
        davinci  &  0.483  &  \textbf{0.885}  &  0.458  &  0.730  \\
        Cohere  &  0.701  &  0.494  &  \textbf{0.939}  &  0.471  \\
        BLOOMz  &  0.486  &  0.555  &  0.487  &  \textbf{0.969}  \\
    \bottomrule
    \end{tabular} }
    \caption{\textbf{Same-domain, cross-generator experiments: train and test on arXiv (single machine-text generator vs human).} Evaluation accuracy (Acc) with respect to the machine generations across five detectors.}
    \label{tab:arxiv}
\end{table}

\begin{table}[t!]
    \centering
    \footnotesize
    \resizebox{0.49\columnwidth}{!}{
        \addtolength{\tabcolsep}{-1pt}
    \begin{tabular}{l  c  c  c c}
    \toprule
        % Test $\rightarrow$ & \multicolumn{4}{c|}{ChatGPT} & \multicolumn{4}{c|}{davinci} & \multicolumn{4}{c|}{Cohere} & \multicolumn{4}{c}{BLOOMz} \\
        Test $\rightarrow$ & ChatGPT & davinci & Cohere & BLOOMz \\
        Train $\downarrow$ & Acc & Acc & Acc & Acc \\
    \midrule
    \multicolumn{5}{c}{\textbf{RoBERTa(base)}} \\
    \midrule
        ChatGPT  &  \textbf{1.000} &  0.974  &  0.990  &  0.995  \\
        davinci  &  0.999  &  \textbf{0.993} &  0.997  &  0.999  \\
        Cohere  &  \textbf{1.000}  &  0.977  &  \textbf{0.998} &  \textbf{1.000} \\
        BLOOMz  &  \textbf{1.000}  &  0.977  &  0.998  &  \textbf{1.000}  \\

    \midrule
      \multicolumn{5}{c}{\textbf{ELECTRA(large)}} \\
    \midrule
        ChatGPT  &  \textbf{0.983} &  0.592  &  0.593  &  0.685  \\
        davinci  &  0.703  &  \textbf{0.956} &  0.494  &  0.595  \\
        Cohere  &  0.927  &  0.517  &  \textbf{0.952} &  0.655  \\
        BLOOMz  &  0.813  &  0.613  &  0.538  &  \textbf{0.987} \\
    \midrule
    \multicolumn{5}{c}{\textbf{LR-GLTR}} \\
    \midrule
        ChatGPT  &  \textbf{0.974}  &  0.850  &  0.929  &  0.813  \\
        davinci  &  0.941  &  \textbf{0.903}  &  0.905  &  0.775  \\
        Cohere  &  0.965  &  0.850  &  \textbf{0.951}  &  0.756  \\
        BLOOMz  &  0.699  &  0.664  &  0.550  &  \textbf{0.910}  \\
    \midrule
    \multicolumn{5}{c}{\textbf{Stylistic}} \\
    \midrule
        ChatGPT  &  \textbf{0.974}  &  0.933  &  0.876  &  0.637  \\
        davinci  &  0.967  &  \textbf{0.965}  &  0.905  &  0.670  \\
        Cohere  &  0.904  &  0.822  &  \textbf{0.942}  &  0.698  \\
        BLOOMz  &  0.537  &  0.537  &  0.540  &  \textbf{0.952}  \\
    \midrule
    \multicolumn{5}{c}{\textbf{NELA}} \\
    \midrule
        ChatGPT  &  \textbf{0.956}  &  0.910  &  0.781  &  0.502  \\
        davinci  &  0.946  &  \textbf{0.925}  &  0.875  &  0.489  \\
        Cohere  &  0.800  &  0.748  &  \textbf{0.938}  &  0.472  \\
        BLOOMz  &  0.494  &  0.492  &  0.496  &  \textbf{0.960}  \\
    \bottomrule
    \end{tabular} }
    \caption{\textbf{Same-domain, cross-generator experiments: train and test on Wikipedia (single machine-text generator vs human).} evaluation accuracy (Acc) with respect to machine generations across five detectors.}
    \label{tab:wikipedia}
\end{table}



==> section/tables/old_tables.tex <==
% \begin{table*}[t!]
%     \centering
%     \small
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{l | ll | ll | ll | ll | ll}
%     \toprule
%         Data Domain $\rightarrow$ & \multicolumn{2}{c|}{Wikipedia} & \multicolumn{2}{c|}{Reddit ELI5} & \multicolumn{2}{c|}{WikiHow} & \multicolumn{2}{c|}{PeerRead} & \multicolumn{2}{c|}{arXiv abstract} \\
%         Models $\downarrow$ & Acc & F1 & Acc & F1 & Acc & F1 & Acc & F1 & Acc & F1 \\
%     \midrule
%         RoBERTa (fine-tuned) \\
%         XLM-R (fine-tuned) \\
%         GLTR LR \\
%         stylometry \\
%         NELA \\
%         authorship attribution\\
%     \midrule
%          GPT0 \\
%          OpenAI detector \\
%     \midrule 
%         Human (50 $\times$ 2) \\
%     \bottomrule
%     \end{tabular} }
%     \caption{\textbf{Train on all domain:} In-domain evaluation accuracy (Acc) and F1 scores(\%) of different models over testsets from different domains. Models are trained using all English training data across domains.}
%     \label{tab:indomaintest}
% \end{table*}

% \begin{table*}[t!]
%     \centering
%     \small
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{l | ll | ll | ll | ll | ll}
%     \toprule
%         Test $\rightarrow$ & \multicolumn{2}{c|}{Wikipedia} & \multicolumn{2}{c|}{Reddit ELI5} & \multicolumn{2}{c|}{WikiHow} & \multicolumn{2}{c|}{PeerRead} & \multicolumn{2}{c|}{arXiv abstract}  \\
%         Train $\downarrow$ & Acc & F1 & Acc & F1 & Acc & F1 & Acc & F1 & Acc & F1 \\
%     \midrule
%         Wikipedia \\
%         Reddit ELI5 \\
%         WikiHow \\
%         PeerRead \\
%         arXiv abstract \\
%     \bottomrule
%     \end{tabular} }
%     \caption{\textbf{Train on a single domain (fill in the top right triangle only):} Out-of-domain evaluation accuracy (Acc) and F1 scores(\%) based on RoBERTa over testsets.}
%     \label{tab:outofdomaintest}
% \end{table*}
